Scalability of High-Performance PDE Solvers

Performance tests and analyses are critical to effective HPC software development and are central components in the design and implementation of computational algorithms for achieving faster simulations on existing and future computing architectures for large-scale application problems. In this paper, we explore performance and space-time trade-offs for important compute-intensive kernels of large-scale numerical solvers for PDEs that govern a wide range of physical applications. We consider a sequence of PDE- motivated bake-off problems designed to establish best practices for efficient high-order simulations across a variety of codes and platforms. We measure peak performance (degrees of freedom per second) on a fixed number of nodes and identify effective code optimization strategies for each architecture. In addition to peak performance, we identify the minimum time to solution at 80% parallel efficiency. The performance analysis is based on spectral and p-type finite elements but is equally applicable to a broad spectrum of numerical PDE discretizations, including finite difference, finite volume, and h-type finite elements.

==> tex/algorithm.tex <==
%%%%%
%%MM: Most of this part is replaced by mathematical formulation at the beginning
%%%%%

%%\subsection{General Algorithm}
%%Finite element operators are typically defined through weak formulations of
%%partial differential equations that involve integration over a computational
%%mesh. The required integrals are computed by splitting them as a sum over the
%%mesh elements, mapping each element to a simple reference element (e.g. the unit
%%square) and applying a quadrature rule in reference space.

%%This sequence of operations highlights an inherent hierarchical structure
%%present in all finite element operators where the evaluation starts on {\em
%%  global (trial) degrees of freedom (dofs)} on the whole mesh, restricts to {\em
%%  degrees of freedom on subdomains} (groups of elements), then moves to
%%independent {\em degrees of freedom on each element}, transitions to independent
%%{\em quadrature points} in reference space, performs the integration, and then
%%goes back in reverse order to global (test) degrees of freedom on the whole
%%mesh.

%%This is illustrated in Figure~\ref{fig_op_decom} for the simple case of
%%symmetric linear operator on third order ($Q_3$) scalar continuous ($H^1$)
%%elements, where we use the notions {\bf T-vector}, {\bf L-vector}, {\bf
%%  E-vector} and {\bf Q-vector} to represent the sets corresponding to the (true)
%%degrees of freedom on the global mesh, the split local degrees of freedom on the
%%subdomains, the split degrees of freedom on the mesh elements, and the values at
%%quadrature points, respectively.

%%We refer to the operators that connect the different types of vectors as:
%%\begin{itemize}
%%\item Subdomain restriction $P$
%%\item Element restriction $G$
%%\item Basis (Dofs-to-Qpts) evaluator $B$
%%\item Operator at quadrature points $D$
%%\end{itemize}
%%More generally, when the test and trial space differ, they get their own
%%versions of $P$, $G$ and $B$.

%%\begin{figure}
%%\begin{center}
%% \includegraphics[width=0.90\textwidth]{./figs/mfem_algorithm.png}
%% \caption{\label{fig_op_decom}Fundamental finite element operator decomposition.}
%%\end{center}
%%\end{figure}
%%
%%\begin{comment}
%%Note that in the case of adaptive mesh refinement (AMR), the restrictions $P$
%%and $G$ will involve not just extracting sub-vectors, but evaluating values at
%%constrained degrees of freedom through the AMR interpolation. There can also be
%%several levels of subdomains ($P_1$, $P_2$, etc.), and it may be convenient to
%%split $D$ as the product of several operators ($D_1$, $D_2$, etc.).
%%\end{comment}
%%
%%\subsubsection{Partial Assembly} \label{sec:pa}
%%Since the global operator $A$ is just a series of variational restrictions with
%%$B$, $G$ and $P$, starting from its point-wise kernel $D$, a ``matvec'' with $A$
%%can be performed by evaluating and storing some of the innermost variational
%%restriction matrices, and applying the rest of the operators ``on-the-fly''. For
%%example, one can compute and store a global matrix on {\bf T-vector}
%%level. Alternatively, one can compute and store only the subdomain ({\bf L-vector}) or
%%element ({\bf E-vector}) matrices and perform the action of $A$ using matvecs with $P$
%%or $P$ and $G$. While these options are natural for low-order discretizations,
%%they are not a good fit for high-order methods due to the amount of FLOPs needed
%%for their evaluation, as well as the memory transfer needed for a matvec.

%%Our focus in Nek5000, MFEM, and deal.II, instead, is on partial assembly, where
%%we compute and
%%store only $D$ (or portions of it) and evaluate the actions of $P$, $G$ and $B$
%%on-the-fly. Critically for performance, we take advantage of the tensor-product
%%structure of the degrees of freedom and quadrature points on quad and hex
%%elements to perform the action of $B$ without storing it as a matrix.
%%

%% MMS: we will look if we can make cloer link to the current BP/BKs.
  \begin{figure}
   \begin{center}
    \includegraphics[width=0.90\textwidth]{./figs/TensorVsAssembly.pdf}
    \caption{\label{fig:TensorVsAssembly}
      Comparison of memory transfer and floating-point operations per
      degree of freedom for different representations of a linear operator for a
      PDE in 3D with $b$ components and variable coefficients arising due to
      Newton linearization of a material nonlinearity.  The ``tensor''
      representation computes metric terms on the fly and stores a compact
      representation of the linearization at quadrature points.  The
      ``tensor-qstore'' representation pulls the metric terms into the stored
      representation.  The ``assembled'' representation uses a (block) CSR
      format.}
   \end{center}
  \end{figure}

%%Implemented properly, the partial assembly algorithm requires optimal amount of
%%memory transfers (with respect to the polynomial order) and near-optimal FLOPs
%%for operator evaluation, see Figure~\ref{fig:TensorVsAssembly}.  It consists of
%%an operator {\em setup} phase, that evaluates and stores $D$ and an operator
%%{\em apply} (evaluation) phase that computes the action of $A$ on an input
%%vector. When desired, the setup phase may be done as a side-effect of evaluating
%%a different operator, such as a nonlinear residual.  The relative costs of the
%%setup and apply phases are different depending on the physics being expressed
%%and the representation of $D$.

%%\subsubsection{Parallel Decomposition}
%%After the application of each of the first three transition operators, $P$, $G$
%%and $B$, the operator evaluation is decoupled on their ranges, so $P$, $G$ and
%%$B$ allow us to ``zoom-in'' to subdomain, element and quadrature point level,
%%ignoring the coupling at higher levels.
%%
%%Thus, a natural mapping of $A$ on a parallel computer is to split the {\bf T-vector}
%%over MPI ranks (a non-overlapping decomposition, as is typically used for sparse
%%matrices), and then split the rest of the vector types over computational
%%devices (CPUs, GPUs, etc.) as indicated by the shaded regions in Figure
%%\ref{fig_op_decom}.
%%
%%One of the advantages of the decomposition perspective in these settings is that
%%the operators $P$, $G$, $B$ and $D$ clearly separate the MPI parallelism in the
%%operator ($P$) from the unstructured mesh topology ($G$), the choice of the
%%finite element space/basis ($B$) and the geometry and point-wise physics $D$.
%%These components also naturally fall in different classes of numerical
%%algorithms -- parallel (multi-device) linear algebra for $P$, sparse (on-device)
%%linear algebra for $G$, dense/structured linear algebra (tensor contractions)
%%for $B$ and parallel point-wise evaluations for $D$.
%%
%%\begin{comment}
%%Currently in libCEED, it is assumed that the host application manages the global
%%{\bf T-vector}s and the required communications among devices (which are
%%generally on different compute nodes) with $P$. Our API is thus focused on the
%%{\bf L-vector} level, where the logical devices, which in the library are
%%represented by the \texttt{Ceed} object, are independent.  Each MPI rank can use
%%one or more \texttt{Ceed}s, and each \texttt{Ceed}, in turn, can represent one
%%or more physical devices, as long as libCEED backends support such
%%configurations. The idea is that every MPI rank can use any logical device it is
%%assigned at runtime. For example, on a node with 2 CPU sockets and 4 GPUs, one
%%may decide to use 6 MPI ranks (each using a single \texttt{Ceed} object): 2
%%ranks using 1 CPU socket each, and 4 using 1 GPU each. Another choice could be
%%to run 1 MPI rank on the whole node and use 5 \texttt{Ceed} objects: 1 managing
%%all CPU cores on the 2 sockets and 4 managing 1 GPU each. The communications
%%among the devices, e.g. required for applying the action of $P$, are currently
%%out of scope of libCEED.  The interface is non-blocking for all operations
%%involving more than $O(1)$ data, allowing operations performed on a coprocessor
%%or worker threads to overlap with operations on the host.
%%\end{comment}

%\end{sm}


==> tex/gpu_old.tex <==
\subsection{Bakeoff problems on GPUs, V100} \label{sec:gpu}

\subsubsection{BK5} \label{sec:gpu_bk5}

Here, we consider the performance of BK5 implemented on an NVIDIA
V100 core on Summit using OCCA (\cite{occa}).
The BK5 performance kernel amounts to evaluating the matrix-vector
product $\uw_L = A_L \uu_L$, where $A_L$=block-diag($A^e$), $e=1,\dots,E$.
This kernel is fully parallel because $A_L$ represents the {\em unassembled}
stiffness matrix using the formulation in (\ref{eq:bk5x}).
 In order to understand
performance tuning on the V100, we presently consider only the kernel (BK5),
not the full miniapp (BP5), which means we are ignoring communication
and device-to-host transfer costs.   Clearly, these issues will be important
in the final analysis.  Communication overhead, however, is well understood
from decades of experience with message-passing implementations of
Nek5000 (e.g., \cite{fisc88,fiscpat94,tufofisc99}).  Our intent here is
to understand the potential and the limits of GPU-based implementations
of the SEM.  We seek to understand what is required to get a significant
fraction of the V100 peak performance in the context of a distributed memory
parallel computing model such as Summit.


%%The BK5 performance kernel amounts to evaluating the matrix-vector
%%product $\uw_L = A_L \uu_L$, where $A_L$=block-diag($A^e$), $e=1,\dots,E$.
%%This kernel is fully parallel because $A_L$ represents the {\em unassembled}
%%stiffness matrix using the formulation in (\label{eq:bk5x}).
%%The geometric factors are diagonal matrices of size $N_q^3 \times N_q^3$.
%%${\bf G}$ is a symmetric tensor, $G_{ij}=G_{ji}$, so only $6N_q^3$ memory
%%reference are required per element, in addition to the $N_q^3$ required
%%to read $\uu^e$.  $\Dh$ requires only $N_q^2$ reads, which are amortized
%%over multiple elements and therefore discounted in the analysis.
%%For $E$ elements, the work complexity for (\ref{eq:bk5e}) is $W \,=\, 12N_q^4
%%\,+\, 15 N_q^3$, with the leading order $O(N_q^4)$ term comprising tensor
%%contractions that can be cast as efficient BLAS3 kernels.
Figure \ref{fig:bk5_tflops_tune} shows the performance for (\ref{eq:bk5e}) on
a single GPU of Summit through a sequence of OCCA tuning steps.  The
number of elements is $E=4096$ and the polynomial order $N$ varies from 1 to 15
($N_q$=2 to 16). Each kernel is run for multiple times and the time for the
kernel is taken by dividing total time by the total number of iterations.
This is done to smooth out the noise and to be sure that we are not misguided
by the clock resolutions on different systems. We note in particular that
$N_q=8$ and 16 see significant performance gains for $K8$.

The tuning curves of Fig. \ref{fig:bk5_tflops_tune} were for the case $E=4096$,
which is the largest we considered.  On leadership class platforms, users are
typically interested in reduced time-to-solution for any given problem (i.e.,
of fixed global size, $n_g$), which means they will increase the node (i.e.,
GPU) count, $P$, to the point where parallel efficiency reaches an intolerable
level (e.g., $<$ 70\%).  Under this strong-scaling scenario, the local number
of points per node, $n=n_g/P$, is reduced.   There is ultimately a point of
marginal return where each GPU lacks sufficient work to keep busy (or to offset
communication).  To understand this strong-scale limit, we performed a sequence
of timings for $E=1,\, 2,\, 4,\,\dots,\,4096$, and analyze the data as a
function of the local number of gridpoints (for a single GPU), $n:=EN^3$.
%% (In the SEM, the number of actual degrees of freedom for an unknown scalar
%% field is typically closer to $EN^3$ than to $EN_q^3$ because of shared degrees
%% of freedom on the element interfaces.)


Figure \ref{fig:bk5_tflops_n} shows the V100 TFLOPS for BK5 as a function
of $n$ for $N=1$ to 15.  The tight data collapse demonstrates that $n$ is a
leading indicator of performance, but the polynomial order is also seen
to be important, with $N=15$ realizing a peak of 2 TFLOPS.  Cursory inspection
of Fig. \ref{fig:bk5_tflops_n} indicates that $n_{\frac{1}{2}}$ for this kernel
is roughly $10^5$, implying that a simulation with $n_g$ points
could realize a speedup of at most $\frac{1}{2} n_g/10^5$ at the 50\% parallel
efficiency level.  We take a closer look at this question in the next two
plots.

Figure \ref{fig:bk5_times} shows the execution time for the cases of Fig.
\ref{fig:bk5_tflops_n}.  The expected linear dependence is evident at the right
side of these graphs while, to the left, the execution time approaches a
constant as $n \longrightarrow 1$.  Interestingly, the execution time in the
linear regime is very weakly dependent on $N$, which typically argues for
larger values of $N$ (and hence more accuracy) and correspondingly smaller
values of $E$ such that the resolution requirements ($n_g$) are met for the
given simulation.  Other considerations, such as meshing or timestep size,
inhibit using excessively high polynomial orders and experience has shown $N=5$
to 9 to be most practical for production simulations.

With this background, deeper insight to the $(N,E,P)$ performance trade-offs
can be gained by looking at the execution time per point, shown in Fig.
\ref{fig:bk5_times_ppt}, which also shows the minimal time and the 2$\times$
line, which is twice the minimal execution time per point.  For a fixed total
problem size, $n_g$, moving horizontally on this plot corresponds to reducing
$n$ and increasing $P$ such that $n_g = P \, n$.  In the absence of (yet to be
included) communication overhead, one gains a full $P$-fold reduction in the
execution if the time per point does not increase when moving to the left.  We
see in this plot that $N=7$ appears to offer the best potential for high
performance, where even at $n=30,000$ the execution time per point is within a
small multiple of the minimum realized over all cases.  This low value of $n$
is in sharp contrast with the $N=14$ and 15 cases, which cross the $2 \times$
line at $n=200,000$.  Thus, through additional inter-node parallelism, the
$N=7$ case affords a potential 200/30 $\approx$ 7-fold performance gain over
the larger $N$ cases.

We note that the conclusion that $N=7$ is superior to $N=15$ in this context
runs contrary to standard intuition, which suggests that, with an $O(N)$
flop-to-byte ratio for (\ref{eq:bk5e}), performance would be best served by
{\em increasing} $N$.  Such a conclusion would in fact be correct in the
saturated limit, where $N$-independent time is seen at the right of the graphs
in Fig. \ref{fig:bk5_times}.  In an {\em HPC} context, however, we are interested
in running problems that are as {\em small as possible on each node}.  We
can see in Fig. \ref{fig:bk5_times} that the low-$N$ curves continue to
trend downward when the large-$N$ curves flatten out as $n$ is reduced.
Thus, in the strong scale limit, a modest value of $N$ proves to be the
most scalable.

Naturally, this analysis needs to be repeated to include other parts of the
Navier-Stokes solver, including host-device transfers and internode
communication, but the analysis approach will be essentially the same.  One
needs to understand where the strong-scale limits are to make informed
discretization and algorithmic choices.

\subsubsection{BP5} \label{sec:gpu_bp5}

\begin{figure} %[!h]
 \centering
 \subfloat[order  6]{{\includegraphics[width=0.33\textwidth]{figs/BP5_t80_06.pdf}}}
 \subfloat[order  8]{{\includegraphics[width=0.33\textwidth]{figs/BP5_t80_08.pdf}}}
 \subfloat[order 10]{{\includegraphics[width=0.33\textwidth]{figs/BP5_t80_10.pdf}}}
  \caption{\label{fig:bp5_nek_libp}BP5 results, time vs DOF/sec of Nek5000 (on BG/Q) and libParanumal (on Summit, V100) for polynomial orders ($p=6, 8, 10$).
\end{figure}


==> tex/intrinsics.tex <==
\section*{Appendix B: Intrinsics on BG/Q}
%GAIL - should not be 11 but B

In this section, we talk about intrinsics on BG/Q that gave a significant
performance boost to MFEM BPs and Nek5000 mxm routines.
Figure~\ref{fig:mfem_intrinsics} shows the results for BP 1, 3, and 5 after
using QPX functions in BG/Q.

Intrinsic functions (or instructions) can be thought of as an intermediate between high-level language
(like C or Fortran) and assembly language. For the IBM PowerPC architecture, these functions are
provided by the QPX (Quad processor extension) to the base IBM POWER instruction set architecture. The
computational model of the QPX architecture is a single instruction, multiple data (SIMD) model with
four execution slots. Each SIMD operation operates on four doubles or floats. Each vector intrinsic
operation maps to a single QPX instruction that can be called from a high-level language.

\begin{figure}
\begin{verbatim}
subroutine mxm_bgq_8(a,n1,b,n2,c,n3)
real(8)  a(n1,8),b(8,n3),c(n1,n3)

vector(real(8)) av1,av2,av3,av4,av5,av6,av7,av8
vector(real(8)) bv1,bsv1,bsv2,bsv3,bsv4
vector(real(8)) bv2,bsv5,bsv6,bsv7,bsv8,cv

call alignx(32, a(1,1))
call alignx(32, b(1,1))
call alignx(32, c(1,1))

do i = 1, n1, 4
  av1 = vec_ld(0,a(i,1))
  av2 = vec_ld(0,a(i,2))
  av3 = vec_ld(0,a(i,3))
  av4 = vec_ld(0,a(i,4))
  av5 = vec_ld(0,a(i,5))
  av6 = vec_ld(0,a(i,6))
  av7 = vec_ld(0,a(i,7))
  av8 = vec_ld(0,a(i,8))

  do j = 1, n3
    bv1  = vec_ld(0,b(1,j))
    bv2  = vec_ld(0,b(5,j))
    bsv1 = vec_splat(bv1, 0)
    bsv2 = vec_splat(bv1, 1)
    bsv3 = vec_splat(bv1, 2)
    bsv4 = vec_splat(bv1, 3)
    bsv5 = vec_splat(bv2, 0)
    bsv6 = vec_splat(bv2, 1)
    bsv7 = vec_splat(bv2, 2)
    bsv8 = vec_splat(bv2, 3)

    cv =  vec_mul (av1, bsv1)
    cv =  vec_madd(av2, bsv2, cv)
    cv =  vec_madd(av3, bsv3, cv)
    cv =  vec_madd(av4, bsv4, cv)
    cv =  vec_madd(av5, bsv5, cv)
    cv =  vec_madd(av6, bsv6, cv)
    cv =  vec_madd(av7, bsv7, cv)
    cv =  vec_madd(av8, bsv8, cv)

    call vec_st(cv, 0, c(i,j))
  enddo
enddo
return
end subroutine mxm_bgq_8
\end{verbatim}
\caption{QPX Intrinsics routine for $C=AB$ with inner-product length 8.
\label{fig:qpx} }
\end{figure}

Shown in Figure B1 is the routine for multiplying matrices $A$ and $B$ where
$A$ is $n_1 \times 8$ and $B$ is $8 \times n_3$ where $n_1$ is divisible by 4.
QPX instructions that map to vector intrinsics are prefixed with $vec\_$. For
example, $vec\_ld$ instruction loads four consecutive double(real(8)) values
into the registers. We can see that $av1, av2, .. av8$ in the above code load a
$4 \times 8$ matrix where $av$'s are the columns.  This matrix can be loaded by
chunks of 4 rows since we assume that $n_1$ is divisible by 4.  Then the $j$th
column of $B$ is split into two and loaded into $bv1$ and $bv2$.  This step is
also possible because we assume that $n_2$ is equal to 8. Then the first value
of $bv1$ is repeated four times in $bsv1$ and so on using $vec\_splat$ routine.
Then $vec\_mul$ and $vec\_madd$ routines perform the matrix-vector
multiplication by multiplying each column of $A$ by relevant $b$ vector value
and summing it up.

%\subsection{MFEM results with intrinsics}

%Figure~\ref{fig:mfem_intrinsics} shows the results for BP 1, 3 and 5 after using
%QPX functions in BG/Q.

\begin{figure}%[!h]
 \begin{center}
 \subfloat[BP1 MFEM]{{\includegraphics[width=0.35\textwidth]{./figs/plot2_MFEM_bp1_v1_cetus_xlc_x86_N512_pn32.pdf}}}
 \subfloat[BP3 MFEM]{{\includegraphics[width=0.35\textwidth]{./figs/plot2_MFEM_bp3_v1_cetus_xlc_x86_N512_pn32.pdf}}}
 \subfloat[BP5 MFEM]{{\includegraphics[width=0.35\textwidth]{./figs/plot2_MFEM_bp5_v1_cetus_xlc_x86_N512_pn32.pdf}}}
 \caption{\label{fig:mfem_intrinsics}BP1, 3, and 5 results of MFEM on BG/Q with varying polynomial order ($p=2,...,14$) with
        intrinsics-based implementation/}
 \end{center}

 \end{figure}


==> tex/performance.tex <==
\subsection{Bakeoff Kernels on GPUs, V100}

Here, we consider the performance of BK5 implemented on an NVIDIA
V100 core on Summit using OCCA (\cite{occa}).
The BK5 performance kernel amounts to evaluating the matrix-vector
product $\uw_L = A_L \uu_L$, where $A_L$=block-diag($A^e$), $e=1,\dots,E$.
This kernel is fully parallel because $A_L$ represents the {\em unassembled}
stiffness matrix using the formulation in (\ref{eq:bk5x}).
 In order to understand
performance tuning on the V100, we presently consider only the kernel (BK5),
not the full miniapp (BP5), which means we are ignoring communication
and device-to-host transfer costs.   Clearly, these issues will be important
in the final analysis.  Communication overhead, however, is well understood
from decades of experience with message-passing implementations of
Nek5000 (e.g., \cite{fisc88,fiscpat94,tufofisc99}).  Our intent here is
to understand the potential and the limits of GPU-based implementations
of the SEM.  We seek to understand what is required to get a significant
fraction of the V100 peak performance in the context of a distributed memory
parallel computing model such as Summit.


%%The BK5 performance kernel amounts to evaluating the matrix-vector
%%product $\uw_L = A_L \uu_L$, where $A_L$=block-diag($A^e$), $e=1,\dots,E$.
%%This kernel is fully parallel because $A_L$ represents the {\em unassembled}
%%stiffness matrix using the formulation in (\label{eq:bk5x}).
%%The geometric factors are diagonal matrices of size $N_q^3 \times N_q^3$.
%%${\bf G}$ is a symmetric tensor, $G_{ij}=G_{ji}$, so only $6N_q^3$ memory
%%reference are required per element, in addition to the $N_q^3$ required
%%to read $\uu^e$.  $\Dh$ requires only $N_q^2$ reads, which are amortized
%%over multiple elements and therefore discounted in the analysis.
%%For $E$ elements, the work complexity for (\ref{eq:bk5e}) is $W \,=\, 12N_q^4
%%\,+\, 15 N_q^3$, with the leading order $O(N_q^4)$ term comprising tensor
%%contractions that can be cast as efficient BLAS3 kernels.
Figure \ref{fig:bk5_tflops_tune} shows the performance for (\ref{eq:bk5e}) on
a single GPU of Summit through a sequence of OCCA tuning steps.  The
number of elements is $E=4096$ and the polynomial order $N$ varies from 1 to 15
($N_q$=2 to 16). Each kernel is run for multiple times and the time for the
kernel is taken by dividing total time by the total number of iterations.
This is done to smooth out the noise and to be sure that we are not misguided
by the clock resolutions on different systems. We note in particular that
$N_q=8$ and 16 see significant performance gains for $K8$.

The tuning curves of Fig. \ref{fig:bk5_tflops_tune} were for the case $E=4096$,
which is the largest we considered.  On leadership class platforms, users are
typically interested in reduced time-to-solution for any given problem (i.e.,
of fixed global size, $n_g$), which means they will increase the node (i.e.,
GPU) count, $P$, to the point where parallel efficiency reaches an intolerable
level (e.g., $<$ 70\%).  Under this strong-scaling scenario, the local number
of points per node, $n=n_g/P$, is reduced.   There is ultimately a point of
marginal return where each GPU lacks sufficient work to keep busy (or to offset
communication).  To understand this strong-scale limit, we performed a sequence
of timings for $E=1,\, 2,\, 4,\,\dots,\,4096$, and analyze the data as a
function of the local number of gridpoints (for a single GPU), $n:=EN^3$.
%% (In the SEM, the number of actual degrees of freedom for an unknown scalar
%% field is typically closer to $EN^3$ than to $EN_q^3$ because of shared degrees
%% of freedom on the element interfaces.)


Figure \ref{fig:bk5_tflops_n} shows the V100 TFLOPS for BK5 as a function
of $n$ for $N=1$ to 15.  The tight data collapse demonstrates that $n$ is a
leading indicator of performance, but the polynomial order is also seen
to be important, with $N=15$ realizing a peak of 2 TFLOPS.  Cursory inspection
of Fig. \ref{fig:bk5_tflops_n} indicates that $n_{\frac{1}{2}}$ for this kernel
is roughly $10^5$, implying that a simulation with $n_g$ points
could realize a speedup of at most $\frac{1}{2} n_g/10^5$ at the 50\% parallel
efficiency level.  We take a closer look at this question in the next two
plots.

Figure \ref{fig:bk5_times} shows the execution time for the cases of Fig.
\ref{fig:bk5_tflops_n}.  The expected linear dependence is evident at the right
side of these graphs while, to the left, the execution time approaches a
constant as $n \longrightarrow 1$.  Interestingly, the execution time in the
linear regime is very weakly dependent on $N$, which typically argues for
larger values of $N$ (and hence more accuracy) and correspondingly smaller
values of $E$ such that the resolution requirements ($n_g$) are met for the
given simulation.  Other considerations, such as meshing or timestep size,
inhibit using excessively high polynomial orders and experience has shown $N=5$
to 9 to be most practical for production simulations.

With this background, deeper insight to the $(N,E,P)$ performance trade-offs
can be gained by looking at the execution time per point, shown in Fig.
\ref{fig:bk5_times_ppt}, which also shows the minimal time and the 2$\times$
line, which is twice the minimal execution time per point.  For a fixed total
problem size, $n_g$, moving horizontally on this plot corresponds to reducing
$n$ and increasing $P$ such that $n_g = P \, n$.  In the absence of (yet to be
included) communication overhead, one gains a full $P$-fold reduction in the
execution if the time per point does not increase when moving to the left.  We
see in this plot that $N=7$ appears to offer the best potential for high
performance, where even at $n=30,000$ the execution time per point is within a
small multiple of the minimum realized over all cases.  This low value of $n$
is in sharp contrast with the $N=14$ and 15 cases, which cross the $2 \times$
line at $n=200,000$.  Thus, through additional inter-node parallelism, the
$N=7$ case affords a potential 200/30 $\approx$ 7-fold performance gain over
the larger $N$ cases.

We note that the conclusion that $N=7$ is superior to $N=15$ in this context
runs contrary to standard intuition, which suggests that, with an $O(N)$
flop-to-byte ratio for (\ref{eq:bk5e}), performance would be best served by
{\em increasing} $N$.  Such a conclusion would in fact be correct in the
saturated limit, where $N$-independent time is seen at the right of the graphs
in Fig. \ref{fig:bk5_times}.  In an {\em HPC} context, however, we are interested
in running problems that are as {\em small as possible on each node}.  We
can see in Fig. \ref{fig:bk5_times} that the low-$N$ curves continue to
trend downward when the large-$N$ curves flatten out as $n$ is reduced.
Thus, in the strong scale limit, a modest value of $N$ proves to be the
most scalable.

Naturally, this analysis needs to be repeated to include other parts of the
Navier-Stokes solver, including host-device transfers and internode
communication, but the analysis approach will be essentially the same.  One
needs to understand where the strong-scale limits are to make informed
discretization and algorithmic choices.

